Control-A-Video: Controllable Text-to-Video Diffusion Models with Motion Prior and Reward Feedback Learning

Recent advances in text-to-image (T2I) diffusion models have enabled impressive image generation capabilities guided by text prompts. However, extending these techniques to video generation remains challenging, with existing text-to-video (T2V) methods often struggling to produce high-quality and motion-consistent videos. In this work, we introduce Control-A-Video, a controllable T2V diffusion model that can generate videos conditioned on text prompts and reference control maps like edge and depth maps. To tackle video quality and motion consistency issues, we propose novel strategies to incorporate content prior and motion prior into the diffusion-based generation process. Specifically, we employ a first-frame condition scheme to transfer video generation from the image domain. Additionally, we introduce residual-based and optical flow-based noise initialization to infuse motion priors from reference videos, promoting relevance among frame latents for reduced flickering. Furthermore, we present a Spatio-Temporal Reward Feedback Learning (ST-ReFL) algorithm that optimizes the video diffusion model using multiple reward models for video quality and motion consistency, leading to superior outputs. Comprehensive experiments demonstrate that our framework generates higher-quality, more consistent videos compared to existing state-of-the-art methods in controllable text-to-video generation

==> mqrpwsnddnxrdszwbbrtshtcmyyqyqvh/sec/0_abstract.tex <==



\begin{abstract}
% This paper presents a controllable text-to-video (T2V) diffusion model, named Video-ControlNet, that generates videos conditioned on a sequence of control signals, such as edge or depth maps. Video-ControlNet is built on a pre-trained conditional text-to-image (T2I) diffusion model by incorporating a spatial-temporal self-attention mechanism and trainable temporal layers for efficient cross-frame modeling. A first-frame conditioning strategy is proposed to facilitate the model to generate videos transferred from the image domain as well as arbitrary-length videos in an auto-regressive manner. Moreover, Video-ControlNet employs a novel residual-based noise initialization strategy to introduce motion prior from an input video, producing more coherent videos. With the proposed architecture and strategies, Video-ControlNet can achieve resource-efficient convergence and generate superior quality and consistent videos with fine-grained control. Extensive experiments demonstrate its success in various video generative tasks such as video editing and video style transfer, outperforming previous methods in terms of consistency and quality.

% Recent advancements in diffusion models have unlocked unprecedented abilities in visual creation. 
% However, current text-to-video generation models struggle with the trade-off among movement range, action coherence and object consistency. 
% To mitigate this issue, we present a controllable text-to-video (T2V) diffusion model, called Control-A-Video, capable of maintaining consistency while customizable video synthesis. 
% Based on a pre-trained conditional text-to-image (T2I) diffusion model, our model aims to generate videos conditioned on a sequence of control signals, such as edge or depth maps. 
% For the purpose of improving object consistency, Control-A-Video integrates motion priors and content priors into video generation: (1) We propose two motion-adaptive noise initialization strategies, which are based on pixel residual and optical flow, to introduce motion priors from input videos, producing more coherent videos.
% (2) We proposed to utilize the first frame generated from T2I model as a content prior to help generates semantic aligned video.

% With the proposed architecture and strategies, our model achieves resource-efficient convergence and generate consistent and coherent videos with fine-grained control. 
% Extensive experiments demonstrate its success in various video generative tasks such as video editing and video style transfer, outperforming previous methods in terms of consistency and quality.



Recent advances in text-to-image (T2I) diffusion models have enabled impressive image generation capabilities guided by text prompts. However, extending these techniques to video generation remains challenging, with existing text-to-video (T2V) methods often struggling to produce high-quality and motion-consistent videos. In this work, we introduce Control-A-Video, a controllable T2V diffusion model that can generate videos conditioned on text prompts and reference control maps like edge and depth maps. To tackle video quality and motion consistency issues, we propose novel strategies to incorporate content prior and motion prior into the diffusion-based generation process. Specifically, we employ a first-frame condition scheme to transfer video generation from the image domain. Additionally, we introduce residual-based and optical flow-based noise initialization to infuse motion priors from reference videos, promoting relevance among frame latents for reduced flickering. Furthermore, we present a Spatio-Temporal Reward Feedback Learning (ST-ReFL) algorithm that optimizes the video diffusion model using multiple reward models for video quality and motion consistency, leading to superior outputs. Comprehensive experiments demonstrate that our framework generates higher-quality, more consistent videos compared to existing state-of-the-art methods in controllable text-to-video generation. 
\keywords{Diffusion Model \and Video Generation \and Feedback Learning}

\end{abstract} 



==> mqrpwsnddnxrdszwbbrtshtcmyyqyqvh/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, the field of text-based visual content generation has witnessed rapid growth.  Current T2I diffusion models \cite{Ramesh_Dhariwal_Nichol_Chu_Chen,saharia2022photorealistic, Rombach_Blattmann_Lorenz_Esser_Ommer_2022} trained on large-scale image-text pairs, showcase impressive capabilities in producing high-quality images guided by user-provided text prompts. Built on these pre-trained T2I models, personalized generation \cite{Ruiz_Li_Jampani_Pritch_Rubinstein_Aberman_2022, gal2022image} and conditional generation \cite{zhang2023adding,mou2023t2i} provide more fine-grained control over the generated image. Further advancements in T2I models have paved the way for personalized generation\cite{Ruiz_Li_Jampani_Pritch_Rubinstein_Aberman_2022, gal2022image} and conditional generation\cite{zhang2023adding, mou2023t2i}, offering finer control over generated videos. The success achieved in image generation has been seamlessly extended to video generation, where Text-to-Video (T2V) diffusion models\cite{singer2022make, ho2022imagen} excel in generating coherent videos driven by text prompts. While some approaches leverage T2I models for one-shot\cite{wu2022tune} or zero-shot\cite{khachatryan2023text2video, qi2023fatezero} video generation, the outcomes often lack consistency or diversity. Other methods\cite{esser2023structure, videocomposer, followyourpose} introduce conditional video generation with control maps, mirroring image-based techniques. 

However, these approaches still grapple with the challenge of producing high-quality and motion-consistent videos.
Concerning video quality, we analyze it from two distinct perspectives: technical quality, characterized by fewer artifacts and reduced blur, and aesthetic quality, gauged subjectively based on human perception of visual appeal. Motion consistency involves both object consistency (where subjects and backgrounds remain unchanged between frames) and motion smoothness (where motion adheres to the principles of physics and no flickering). 

\begin{figure}[t]
\centering
  \includegraphics[width=0.95\linewidth]{./figures/head}%\vspace{-0.4em}
\caption{Our model generates high-quality and consistent videos conditioned on a text prompt and additional control maps, such as \textcolor{red}{depth maps} (first row), \textcolor{cyan}{canny edge maps} (second row), \textcolor{green}{hed edge maps} (third row). }
\label{fig:head} 
\vspace{-0.5cm}
\end{figure}%


In response to the aforementioned challenges, we presents a controllable T2V model, namely Control-A-Video, capable of generating based on text and reference control maps, such as edge, depth maps, as shown in Figure \ref{fig:head}. 
We develop our video generative model by reorganizing a pretrained controllable T2I model \cite{zhang2023adding}, incorporating additional trainable temporal layers, and utilizing a spatial-temporal self-attention mechanism that facilitates fine-grained interactions between frames. This meticulous architectural design, coupled with the incorporation of control signals, notably preserves motion smoothness. 
Furthermore, we propose novel strategies to introduce content prior and motion prior for diffusion-based generation, boosting motion consistency. Additionally, we introduce ST-ReFL, an algorithm that utilizes multiple reward models to enhance both motion consistency and video quality.

For the content prior, we introduce an training scheme that produces video predicated on the initial frame. With this, it becomes more manageable to disentangle content and temporal modeling. Instead of learning the generation of entire videos, our model focuses on generating subsequent frames with content prior derived from the first frame. This design inherits generative capabilities from the image domain, ensuring consistency with objects in the initial frame.
During inference, we employ a Text-to-Image-to-Image-to-Video (T2I-I2V) pipeline. This involves generating an image and using it as a content prior for video generation.
Meanwhile, another benefit of such strategy is that our model can auto-regressively generate a longer video by treating the last frame of the previous iteration as the initial frame. 

The motion prior come from two types of pioneering noise initialization approaches. 
The first method is to initialize noise based on pixel residual between frames of the source video. 
The second one is to calculate the initial noise of next frame based on optical flow of the source video movement. 
Inspired by \cite{preserve}, these approaches can make the initial distribution of noise latents more reasonable, enhancing relevance among frame latents and improving video consistency. 
By leveraging motion prior, the Control-A-Video is able to closely resemble motion changes in the reference video and produce coherent videos that are less flickering and object consistent. 

While prior contribute to enhancing consistency, the denoising training process encounters challenges in learning to generate high-quality videos. These challenges may manifest as aesthetic issues, artifacts, and object inconsistency, as shown in the lower part of Figure \ref{fig:pipeline}. One potential solution lies in leveraging large-scale and high-quality video datasets. Instead of opting for conventional engineering's approaches, such as manually collecting more data, we present an pioneering solution: introducing ST-ReFL algorithm to enhance the video diffusion model by leveraging diverse reward models can score frame-wise video quality and temporal motion consistency. Utilizing rewards from the reward models, we use ST-ReFL algorithm to optimize the diffusion model. This targeted optimization process is designed to boost the overall reward, leading to enhanced quality and consistency in the model's output. Through the implementation of the ST-ReFL training process, our experiments reveal a noticeable reduction in artifacts, improved aesthetic appeal, and heightened consistency in the generated videos. 

In summary, our contributions can be outlined as follows:
(i) \textbf{Control-A-Video Model}: We introduce Control-A-Video, a controllable Text-to-Video diffusion model designed for video generation based on text prompts and reference control maps.
(ii) \textbf{Content prior}: we propose a novel approach, utilizing the first frame as content prior, making it more manageable to disentangle content and temporal modeling during training. During inference, a T2I-I2V pipeline is employed to transfer text-aligned knowledge from images to videos and enabling auto-regressive generation for extended videos.
(iii) \textbf{Motion prior}: We introduce innovative noise initialization strategies, incorporating both pixel residual-based and optical flow-based approaches. These motion prior, derived from reference videos, significantly enhance the relevance among frame latents, resulting in videos that are more consistent with reduced flickering.
(iv) \textbf{ST-ReFL for Video Diffusion Model}: Addressing inefficiency in denoising training, we propose a ST-ReFL algorithm, which leverages diverse reward models to optimize the trained video diffusion model by scoring its output, leading to improvements in both quality and consistency. To the best of our knowledge, we are the first to introduce feedback learning for optimizing video generation model. (v) Comprehensive experiments showcase that our framework excels in generating higher-quality and consistent videos, achieving state-of-the-art results in controllable text-to-video generation. 

% (ii) We introduce pixel residual-based and optical flow-based noise initialization strategies, that incorporate motion prior from the reference videos to promote relevance among frame latents, making videos more consistent and less flickering. 
% (iii) To achieve further object consistency, we also present a novel first-frame conditioned controller to introduce content prior. 
% Our model generates videos based on semantics of the initial frame, transferring text-aligned knowledge from images to videos. 
% As a byproduct of the first-frame conditioning strategy, Control-A-Video can auto-regressively generate longer videos.  


% In recent years, there has been a rapid development in text-based visual content generation. Driven by the progress of diffusion-based models, text-to-image synthesis~\cite{GLIDE, Ramesh_Dhariwal_Nichol_Chu_Chen, saharia2022photorealistic} has demonstrated an impressive ability to generate high-quality images based on user-provided text prompts. 

% Built on pre-trained T2I models, there is a surging interest in text-to-video synthesis in zero-shot manner~\cite{qi2023fatezero, khachatryan2023text2video,renderavideo} or training on large-scale video-text datasets~\cite{esser2023structure,alignyourlatent}. 
% However, movement generation across video frames remains a formidable challenge. 
% A satisfactory generated videos should fulfill three criteria: 
% 1) a distinct range of movement, 2) coherent action during inter-frame transitions, 3) consistent appearance of objects in different frames without flickers. 


% The current T2V models tend to generate videos with limited movement range due to the trade-off among movement range, action coherence and object consistency, as shown in Figure~\ref{fig:motivation}(a). 
% When the motion range is large, consistency and coherence are difficult to maintain. 
% To enhance video movements, the introduction of control signals during video generation is a potential solution. 
% Controllable video synthesis~\cite{videocomposer, makeyourvideo} allows users to specify desired contents and motions, realizing customized video generation with fine-grained control. 

% Nevertheless, despite achieving controllable movements and coherent action, a notable challenge remains in ensuring object consistency. 
% For instance, Figure~\ref{fig:motivation}(b) depicts that the appearance of horse changes across frames, although the motion is correct. 



% \begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.98\linewidth]{./figures/motivation1}
%    \caption{The prompt for generation is ``magical flying horse with a man jumping over an obstacle, artstation''. (a) Text-to-video model\protect\footnotemark[1], (b) Controllable text-to-video baseline\protect\footnotemark[2], (c) Our Control-A-Video model. The result from text-to-video model\protect\footnotemark[1] has only a limited movement range. Baseline controllable generation\protect\footnotemark[2] can create videos with desired movements under the control signals, but it loses consistency. In contrast, our model is capable of maintaining object consistency in customizable video synthesis.}
%    \label{fig:motivation}
%    \vspace{-0.4cm}
% \end{figure}

% \footnotetext[1]{We use the api on https://www.genmo.ai/.}
% \footnotetext[2]{We train the baseline with only depth map condition.}




% With the above strategies, controllable generation results have better consistency like in Figure~\ref{fig:motivation}(c). 
% Moreover, our model is easy to converge with fewer training resources, e.g., our iteration samples are 1.6M compared to 115M in Gen-1's \cite{esser2023structure}.


\section{Related Work}
\subsection{Text-to-image generation with diffusion models}

Over the past few years, significant advancements have been made in image generation, notably with Denoising Diffusion Probabilistic Models (DDPMs) \cite{Ho_Jain_Abbeel_2020,Song_Meng_Ermon_2020}. DDPMs have surpassed the performance of Generative Adversarial Networks (GANs) \cite{goodfellow2020generative} and Variational Autoencoders (VAEs) \cite{vae2013}. To generate images conditioned on text, several approaches like GLIDE \cite{GLIDE}, DALLE-2 \cite{Ramesh_Dhariwal_Nichol_Chu_Chen}, Imagen \cite{saharia2022photorealistic}, and Latent Diffusion Models (LDMs) \cite{Ramesh_Dhariwal_Nichol_Chu_Chen} have been proposed, training diffusion models on large-scale text-image pairs. For personalized generation, few-shot tuning methods such as Textual Inversion \cite{gal2022image} and Dreambooth \cite{Ruiz_Li_Jampani_Pritch_Rubinstein_Aberman_2022} have been developed. Editing techniques like Prompt2Prompt \cite{hertz2022prompt}, Plug-and-Play \cite{tumanyan2022plug}, and InstructPix2Pix \cite{brooks2022instructpix2pix} offer ways to refine generated images. Notably, ControlNet \cite{zhang2023adding}, T2I-Adapter \cite{mou2023t2i}, and Composer \cite{composer} focus on fine-tuning text-to-image (T2I) models with condition-text-image pairs, enabling the integration of control hints like edges, poses, and depth maps. In this paper, we adopt a similar idea to ControlNet and extend it to video generation with conditions. Recently, Reward Feedback Learning approaches have been introduced in the diffusion domain, such as ImageReward \cite{imagereward}, RAFT \cite{RAFT}, and DPOK \cite{DPOK}, demonstrating a promising path to optimize diffusion models. Our work focuses on utilizing reward models to optimize video diffusion models.

\subsection{Text-to-video generation with diffusion models}

The success of diffusion models in text-to-image (T2I) generation has inspired research into video generation. Notable works like VDM \cite{ho2022video}, Imagen Video \cite{ho2022imagen}, Make-A-Video \cite{singer2022make}, and Animatediff \cite{animatediff} extend T2I diffusion models by training on large text-video datasets. To generate longer videos, LVDM \cite{lvdm}, MCVD \cite{mcvd}, and Align-Your-Latents \cite{alignyourlatent} adopt an auto-regressive approach, sequentially generating frames for temporal coherence.

For text-based video translation, zero-shot methods such as Text2Video-Zero \cite{khachatryan2023text2video}, FateZero \cite{qi2023fatezero}, Vid2VidZero \cite{vid2vid-zero}, and Video-P2P \cite{vid-p2p} explore diffusion model latent spaces and employ temporal attention, but may lack temporal consistency. To improve consistency, flow-based approaches like Render-A-Video \cite{renderavideo} and TokenFlow \cite{tokenflow} introduce flow constraints, while tuning-based methods like Tune-A-Video \cite{wu2022tune} and CodeF \cite{codef} fine-tune models during inference, albeit requiring additional tuning. Gen-1 \cite{esser2023structure} and VideoCompose \cite{videocomposer} train video diffusion models with conditional maps. In contrast, this paper presents a novel two-stage generation approach (T2I-I2V) and employs noise manipulation to enhance temporal consistency in text-based video translation. Besides, we propose to use ST-ReFL to improve video quality and consistency.

% The remarkable accomplishments of diffusion models in Text-to-Image (T2I) generation have inspired researchers to venture into the field of video generation. Several notable advancements, including VDM \cite{ho2022video}, Imagen Video \cite{ho2022imagen}, Make-A-Video \cite{singer2022make} and Animatediff \cite{animatediff}, extend text-to-image diffusion models by training them on extensive text-video pairs. To overcome the challenge of generating longer videos, LVDM \cite{lvdm}, MCVD \cite{mcvd}, and Align-Your-Latents \cite{alignyourlatent} adopt an auto-regressive approach, sequentially generating video frames to ensure temporal coherence and continuity.
% For text-based video translation, zero-shot methods such as Text2Video-Zero \cite{khachatryan2023text2video}, FateZero \cite{qi2023fatezero}, Vid2VidZero \cite{vid2vid-zero}, and Video-P2P \cite{vid-p2p}, explore the latent space of diffusion models and employ temporal attention mechanisms to generate videos. However, a challenge faced by these methods is the potential lack of temporal consistency.To improve the consistency of the generated videos, flow-based approaches like Render-A-Video \cite{renderavideo} and TokenFlow \cite{tokenflow}propose to introduce flow constraints in diffusion process. On the other hand, tuning-based methods, such as Tune-A-Video \cite{wu2022tune} and CodeF \cite{codef}, achieve better consistency by fine-tuning the models in the inference stage, albeit requiring an additional tuning process. Furthermore, Gen-1 \cite{esser2023structure}, VideoCompose \cite{videocomposer} propose to train video diffusion models with additional conditional maps. In comparison to these existing approaches, this paper presents a novel two-stage generation approach and employs a noise manipulation strategy to achieve enhanced temporal consistency in text-based video translation.


% In recent years, there has been a rapid development in text-based visual content generation. Trained with large-scale image-text pairs, current T2I diffusion models \cite{Ramesh_Dhariwal_Nichol_Chu_Chen,saharia2022photorealistic, Rombach_Blattmann_Lorenz_Esser_Ommer_2022} have demonstrated an impressive ability to generate high-quality images based on user-provided text prompts. Built on these pre-trained T2I models, personalizing generation \cite{Ruiz_Li_Jampani_Pritch_Rubinstein_Aberman_2022, gal2022image} and conditional generation \cite{zhang2023adding,mou2023t2i} provide more fine-grained control over the generated videos. Success in image generation has also been extended to video generation. Some methods leverage T2I models to generate videos in one-shot \cite{wu2022tune} or zero-shot \cite{khachatryan2023text2video, qi2023fatezero} manner, while videos generated from these models are still inconsistent or lack variety. Scaling up video data, text-to-video (T2V) diffusion models \cite{singer2022make,ho2022imagen} are able to generate consistent videos with text prompts, but these models generate videos in a fully automatic way, lacking control over the generated content. A recent study \cite{esser2023structure} propose a T2V diffusion model that allow for depth maps as control. However, a large-scale dataset is required to achieve consistency and high quality, which is resource-unfriendly. Additionally, it's still challenging for T2V diffusion models to generate videos of consistency, arbitrary length and diversity.

% To address these issues, this paper presents a controllable T2V model, namely Control-A-Video, which has the following advantages: (i) Improved consistency: Control-A-Video employs motion prior and control maps to achieve better consistency.  (ii) Generation of videos with arbitrary length: by adopting the proposed first-frame conditioning strategy, Control-A-Video can auto-regressively generate videos of any length. (iii) Domain generalization: the model generates succeeding videos based on the initial frame, transferring knowledge  from images to videos. 
% % videos that go beyond the boundaries of the video domain. 
% (iv) Resource-efficient: our model is easy to converge with fewer training resources. e.g. , our batch size*steps are 16*10k compared to 1152*100k in Gen-1's \cite{esser2023structure}.

% Specifically, the Control-A-Video is designed to generate videos based on text and reference control maps. In terms of model architecture, we develop our video generative model by reorganizing a pre-trained controllable T2I model \cite{zhang2023adding}, incorporating additional trainable temporal layers, and presenting a spatial-temporal self-attention mechanism that facilitates fine-grained interactions between frames. This approach allows for the creation of content-consistent videos, even without extensive training. To ensure video structure consistency, we propose a pioneering approach that incorporates the motion prior of the source video into the denoising process at the noise initialization stage. By leveraging motion prior and control maps, the Control-A-Video is able to produce videos that are less flickering and closely resemble motion changes in the input video, while also avoid error propagation in other motion-based methods \cite{ebsynth2019} due to the nature of multi-step denoising process.
% % , resulting in superior quality outputs.

% % Additionally, the nature of multi-step denoising process corrects potential error propagation in other motion-based methods such as \cite{ebsynth2019}, resulting in superior quality and consistent video outputs.

% Furthermore, instead of previous methods that train models to directly generate entire videos, we introduce an innovative training scheme that produces video predicated on the initial frame. With such a straightforward yet effective strategy, it becomes more manageable to disentangle content and temporal learning, since the former is presented in the first frame and the text prompt. Our model only needs to learn how to generate subsequent frames, inheriting generative capabilities from the image domain and easing the demand for video data. During inference, we generate the first frame conditioned on the control map of the first frame and a text prompt. Then, we generate subsequent frames conditioned on the first frame, text, and subsequent control maps. Meanwhile, another benefit of such strategy is that our model can auto-regressively generate an infinity-long video by treating the last frame of the previous iteration as the initial frame.

% In summary, our contributions can be outlined as follows:
% \begin{itemize}
% \item We propose a controllable T2V diffusion model, named Control-A-Video, by refactoring a controllable T2I model. Our model is able to generate text-guided videos conditioned on various types of control maps.
% \item We introduce a residual-based noise initialization strategy that incorporates motion from the input video into the diffusion process, resulting in the generation of videos that are less flickering and motion-aligned.
% \item We present a novel first-frame conditioning strategy that not only empowers our model to generate videos generalized from the image domain but also to generate arbitrary-length videos auto-regressively.
% \item Experiments demonstrate that our framework is capable of generating higher-quality, more consistent videos using fewer training resources.
% \end{itemize}

==> mqrpwsnddnxrdszwbbrtshtcmyyqyqvh/sec/2_method.tex <==

\begin{figure*}[!t]
   \centering
   \includegraphics[width=0.98\linewidth]{./figures/pipeline3}
   % \caption{Illustration of our Control-A-Video pipeline. \textbf{Model Architecture:} We apply spatial-temporal self-attention and trainable temporal layers to both the image UNet and the image ControlNet, enabling the model to generate videos. \textbf{Training:} The model input includes video and its text prompt from BLIP captioning \cite{BLIP} and control maps from an annotator (e.g. depth estimation model). Each frame is passed to the encoder to get the latent code. We add noise with motion prior to each latent except for the first frame and train the model to predict the subsequent noise conditioned on the first frame. \textbf{Inference:} After training, our model is able to generate the first frame conditioned on its control map. The generated first frame is then used to generate subsequent frames with the content prior.}
   % \caption{Illustration of our Control-A-Video pipeline without feedback learning. \textbf{Model Architecture:} Spatial-temporal self-attention and trainable temporal layers are applied to the image UNet and the image ControlNet. \textbf{Training:} The model input includes video and its text prompt from BLIP captioning \cite{BLIP} and control maps from an annotator (e.g. depth estimation model). We add noise with motion prior to each latent except for the first frame and train the model to predict the subsequent noise conditioned on the first frame. \textbf{Inference:} After training, our model Adopt a T2I-I2V pipeline to generate a video with the content prior. \textbf{Reward Feedback Learning for video generation}: Overview of direct reward feedback optimizing algorithm. The process involves sampling $x_T$ and denoising it to $x_{t+1}$ without gradients. Subsequently, we denoise $x_{t+1}$ to $x_{t}$, decode it, and compute quality and motion rewards. These rewards are then utilized to optimize the diffusion model. The optimization targets include enhancing aesthetic and technical quality (reducing artifacts) and ensuring motion (temporal consistency), as illustrated in the lower-left corner.}

   \caption{\textbf{Illustration of the Control-A-Video pipeline.} \textbf{Architecture:} Spatial-temporal self-attention and trainable temporal layers are applied to the UNet and ControlNet.(Temp denotes Temporal). \textbf{(1) Noise Prediction Training:} We add motion-aware noise to video latents (except the first frame) and train the model to predict the subsequent noise conditioned on the first frame, control maps, and text prompt. \textbf{(2)ST-ReFL Training:} A reward feedback loop optimizes the video diffusion model using (Aesthetic and Technical) Quality and Motion Rewards. It involves sampling $x_T$, denoising to $x_{t+1}$ without gradients, where $t \in [T_1,T_2] $, then denoising $x_{t+1}$ to $x_t$ with gradients to predict $x_0'$, which is decoded and scored by the reward models. The optimization aims to enhance aesthetic and technical quality while ensuring temporal consistency.}
   
   \label{fig:pipeline}
   \vspace{-0.2cm}
\end{figure*}
\vspace{-0.3cm}
\section{Method}

In this section, we will first introduce the controllable video diffusion model and its training and inference process with the first-frame condition scheme. Next, we introduce the motion-adaptive noise prior that help to improve the frame consistency. At the last section, we illustrate the reward feedback learning for video diffusion model that further enhances the capability of our model. 

\subsection{Video Diffusion Model with Control}
\label{architecture}
\textbf{Model Architecture:} Our model is built upon image diffusion model LDMs \cite{Ho_Jain_Abbeel_2020} and ControlNet \cite{zhang2023adding}, where both extra trainable motion layers are applied to UNet and ControlNet for temporal modeling. Similar to other work\cite{singer2022make, esser2023structure}, we add an additional 1D temporal layer to each 2-dimensional (2D) layer, including convolution and attention layers. To further enhance frame modeling, we employ a spatial-temporal self-attention mechanism, where spatial and temporal relationships are jointly model to capture dependencies across frames. 
As shown in Figure \ref{fig:pipeline}, each frame's are processed through either a 2D convolution layer or a spatial attention layer. Subsequently, these frame-level features are collectively passed to a trainable 1D convolutional layer or temporal attention for frame modeling. Moreover, to enable fine-grained modeling, we adapt the spatial self-attention mechanism by incorporating spatial-temporal self-attention across frames, which can be formulated as:

\begin{equation}\label{eq:SelfAttn}
SelfAttn(Q, K, V ) = Softmax(\frac{QK^T}{\sqrt{d}})V ,
\end{equation}
\begin{equation}\label{eq:KQV}
Q = W^Q \bar{v}_i, K = W^K [\bar{v}_0,...,\bar{v}_{N-1}], V = W^V [\bar{v}_0,...,\bar{v}_{N-1}]
\end{equation}
where $\bar{v}_i$ denotes the token sequence of frame $i$, and $[\bar{v}_0,...,\bar{v}_{N-1}]$ denotes the concatenation of the $N$ frames.
As shown in Eq. \ref{eq:KQV}, we concatenate features $K,V$ of $N$ frames so that each position has a global perception of all video frames and tends to generate more consistent results.

% After we get the  $K, V$ matrix with the original parameters $W^K$ and $W^V$ , we apply the same operation as the original self-attention (Eq. \ref{eq:SelfAttn}). 


%\begin{wrapfigure}{lT}{0.5\textwidth}

%\end{wrapfigure}

% \end{figure}


\label{training}
\textbf{Training with content prior:} To inherit the knowledge from image domain, we propose to introduce first frame as content prior to help generate more generalized videos. Specifically, as shown in the upper part of Figure \ref{fig:pipeline}, we add noise to each frames except the first one, and the model learns to denoise the noise with the content prior. This approach reduces the need for the model to memorize video content in the training set and instead focuses on learning to reconstruct motion, which makes it possible to achieve better results with fewer training resources. We thus train the model with the formulated loss function: 
\begin{equation}
min_\theta || \epsilon - \epsilon_\theta(x_t, t, c_p, c_f, \mathcal{E}(v^1)) ||_2^2
\end{equation}
, where $\epsilon$ is the ground truth noise and the diffusion model $\theta$ predict the noise with input $x_t$ at time step $t$ based on conditions prompt $c_p$, control maps $c_f$ and the first frame $v^1$. This simple yet effective strategy not only allows the model learns to effectively utilize the motion information from the control maps and follow the content from the first frame, but also able to auto-regressively generate longer videos. 

\textbf{T2I-I2V inference:} We generate the initial frame, $v^1$, by providing the model with gaussian noise of a single frame $x^1$ along with conditioning factors including a text prompt $c_p$ and a first frame control map $c_f^1$:
\begin{equation}
v^1 = ControlT2I(x^1 , c_p, c_f^1).
\end{equation}
Then we generate the following frames from gaussian noise $x$, where the first frame latent $x^1$ is $\mathcal{E}(v^1)$ from T2I model:
\begin{equation}
v = ControlT2V(x , c_p, c_f, \mathcal{E}(v^1)).
\end{equation}
With our proposed method of first-frame conditioning, our model is capable of generating video sequences with greater diversity than what is present in the training data. Additionally, our model has a distinct advantage in creating longer videos by utilizing previously generated frames as the initial frame in the subsequent iteration. This allows us to use an auto-regressive approach to produce longer videos.
% which sets us apart from other video diffusion models that are limited to generating videos only once.


\textbf{Classifier-Free Guidance}:
% Classifer-free guidance \cite{Ho_Salimans} with a guidance scale $\omega_t$ to sample the noise can be formulated as:
% The noise sampling algorithm used in our diffusion model is classifier-free and involves the use of guidance scales to generate high-quality results.
% \begin{equation}
% \hat{\epsilon}_\theta(x_t, t, c_p, c_f) = \epsilon_\theta(x_t, t, \emptyset, c_f) 
% +\omega_t(\epsilon_\theta(x_t, t, c_p, c_f) - \epsilon_\theta(x_t, t, \emptyset, c_f)) 
% \end{equation}
% \begin{equation}
% \begin{aligned}
% \hat{\epsilon}_\theta(x_t, t, c_p, & c_f) = \epsilon_\theta(x_t, t, \emptyset, c_f) \\
% &+\omega_t(\epsilon_\theta(x_t, t, c_p, c_f) - \epsilon_\theta(x_t, t, \emptyset, c_f)) 
% \end{aligned}
% \end{equation}
% where $\emptyset$ denotes a null-text prompt, and $\epsilon_\theta(x_t, t, \emptyset, c_f)$ represents negative representation.
Based on typical Classifer-free guidance \cite{Ho_Salimans}, we incorporate a sampling strategy in \cite{esser2023structure} that treats noise prediction of video generated frame-by-frame as a negative representation needed to be avoided. Consequently, the final prediction of noise is calculated as:
\begin{equation}
\begin{aligned}
\hat\epsilon_\theta(x_t, t, c_p, c_f) = &\epsilon_{\theta I}(x_t, t, \emptyset, c_f)+\omega_v(\epsilon_\theta(x_t, t, \emptyset, c_f) - \epsilon_{\theta I}(x_t, t, \emptyset, c_f)) \\
&+\omega_t(\epsilon_\theta(x_t, t, c_p, c_f) - \epsilon_\theta(x_t, t, \emptyset, c_f)).
\end{aligned}
\label{eqn:equation}
\end{equation}
Here, $\omega_v$ and $\omega_t$ denote the scales of video guidance, $\emptyset$ denotes a null-text prompt, and $\epsilon_{\theta I}(x_t, t, \emptyset, c_f)$ denotes the prediction that each video frame is independently predicted. Just as a larger $w_t$ can enhance text guidance, a larger $w_v$ will result in a smoother overall effect.



% \begin{wrapfigure}{r}{0.48\textwidth}
%     \centering
%     \includegraphics[width=0.48\textwidth]{./figures/noise_prior2}
%     \caption{\textbf{Motion-adaptive Noise Prior}: we visualize the t-SNE plot of the noisy latents of video frames. The red one denotes the video $X_0$, we gradually add noise from timesteps 0 to 999. The pink one is residual noise, the orange one is flow noise, the green one is gaussian noise. There're two fingings in this map: (1) Two adjacent frames are the most similar, so a sequence of frames should be linked with a line. (2) For gaussian noise, the ``line'' relation is distored and each dot become away from the origin video; for flow-based noise and residual-based noise, the ``line'' is still parallel to the origin frames and the distance is not far away the $X_0$.}
%     \label{fig:vis_noise}
% \end{wrapfigure}


\subsection{Motion-adaptive Noise Prior}
\label{noise_init}
The diffusion model aims to denoise a signal by learning from Gaussian noise, where different initial noise samples can yield different results. In our study, we leverage the components of T2I models for video generation and observe that the latent spaces of consecutive video frames exhibit high correlation.
In Figure \ref{fig:vis_noise}, we can see that consecutive frames (represented by red points) are close to each other. However, when we add per-frame typical Gaussian noise (represented by green points) to each frame, we observe that the distribution between frames is disrupted. Not only does the distance between frames increase, but the overall distribution across frames also becomes distorted. Motivated by these findings, we propose a strategy to incorporate motion into the noise initialization process, aiming to align the noise closer to the video frames. To achieve this, we introduce two types of motion prior for video generation: flow-based and residual-based. By integrating motion-based noise into the latent space of the video, we empirically observe that the distribution of each frame maintains its similarity and coherence. As depicted in Figure \ref{fig:vis_noise}, the distribution of the flow-based noise (represented by orange points) is most similar to the original video, while the residual-based noise (represented by pink points) also exhibits high correlation. Intuitively, learning to reconstruct the video from motion-based noise is more feasible compared to using Gaussian noise since the latent similarity is preserved.
Specifically, the proposed algorithm is outlined in Algorithm \ref{algorithm}.

\begin{wrapfigure}{r}{0.49\textwidth}
\vspace{-23pt}
\setlength{\belowcaptionskip}{-19pt}
    \centering
    \includegraphics[width=0.48\textwidth]{./figures/noise_prior2}
    \caption{\textbf{Motion-adaptive Noise Prior}: t-SNE plot of noisy latents for video frames. Red: original video $X_0$. Noise is gradually added from timesteps 0 to 999, with pink: residual noise, orange: flow noise, green: Gaussian noise. Adjacent frames are linked, showing (1) frame similarity and (2) flow/residual noise preserves the line structure better than Gaussian noise, indicating improved consistency.}
    \label{fig:vis_noise}
\end{wrapfigure}

\textbf{Residual-based Noise Prior:} To maintain consistent noise in static regions and introduce varying noise in moving regions, we employ a residual-based noise prior. By computing the pixel residual between consecutive frames, we initialize the noise distribution accordingly after downsampling. This approach ensures that unchanged areas exhibit the same noise, while changing areas possess distinct noise patterns. Additionally, a threshold is utilized to differentiate static and dynamic regions, providing control over the smoothness of the generated videos.

\textbf{Flow-based Noise Prior:} In order to align the generated video's flow with the motion depicted in the frames, we introduce a flow-based noise prior. This involves computing the optical flow between consecutive frames in pixel space, followed by downsampling the flow information to the latent space. By propagating the flow through subsequent noise latents, we align the noise patterns with the expected motion flow, resulting in visually coherent and realistic videos.


\begin{figure}[t]
  \centering
  \scriptsize
  \begin{minipage}[t]{0.48\textwidth}
    \begin{algorithm}[H]
      \caption{\small Motion-adaptive Noise Propagation}
\label{algorithm}
\textbf{Notations:} Initialize noise $x$ with $N$ frames, $x^n \leftarrow \mathcal{N}(0, I) , n=0,...,(N-1) $ 
Input Video $: v = [ v^n, n=0,...,(N-1) ] $ 
$R_{thres}$ : Threshold for residual change 
% $DownSample()$ : Downsample to noise's dim 

% ---

\textbf{residual-based}

\For{ i from 1 to N}{
$ res = norm( v^i - v^{(i-1)} ) $ \\
$ res_{mask} = res > R_{thres} $ \\    
$res_{mask}$ = $DownSample(res_{mask})$ \\
$x^i = [x^i - x^{(i-1)} ]* res_{mask} +  x^{(i-1)}$ \\
}
% ---

\textbf{flow-based}

\For{ i from 1 to N}{
$ flow^i_{pixel} = flow( v^i , v^{(i-1)} ) $ \\
$ flow^i_{latent} $ = $DownSample(flow_{pixel})$ \\
$ x^i = GridSample(x^{(i-1)}, flow^i_{latent})$ \\ % gridsample?
}
    \end{algorithm}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.49\textwidth}
    \begin{algorithm}[H]
      \caption{\small Spatial-Temporal Reward Feedback Learning for Video Diffusion Models}
\label{algorithm_rlhf}
\textbf{Notations:} Video diffusion model $w$, quality reward model $R_q$, motion reward $R_m$. Total scheduler time steps $T$, randomly sampled timestep $t \in [T1, T2] $. Input latent $x$, output latent $x'$. $\alpha$ is the learning rate. \\
t $\gets$ rand(T1,T2) \\ 
$x_T$ $\sim$ $\mathcal{N}(0, I)$ \\
with no grad:  \\
\For{ i from T to t+2}{ 
$x_{i-1}$ $\gets$ $w(x_i)$ \\
}
with grad: $x_{t}$ $\gets$ $w(x_{t+1})$ \\
$x_0'$ $\gets$ $x_t$  \quad  // predict \\
$v_0'$ $\gets$ $x_0'$, $v_0$ $\gets$ $x_0$   \quad // decode   \\
$L_{motion}$ $\gets$ $R_{m}(v_0, v_0')$, $L_{quality} \gets R_{q}(v_0')$ \\
$\mathcal{L}_{ST} \gets L_{motion} + L_{quality}$ \\
$\Delta \gets \frac{\partial \mathcal{L}_{ST}}{\partial w}$ \\
$w'$ $\gets$ w - $\alpha$ $\Delta$  \quad // update 
    \end{algorithm}
  \end{minipage}
  \vspace{-0.5cm}
\end{figure}

% \begin{algorithm}[!t]
% \caption{Motion-adaptive Noise Propagation}
% \label{algorithm}
% Initialize noise $x$ with $N$ frames, $x^n \leftarrow \mathcal{N}(0, I) , n=0,...,(N-1) $ \\

% % $InputNoise: x =  x^n \leftarrow \mathcal{N}(0, I), n=0,...,(N-1) $ \\
% Given InputVideo $: v = [ v^n, n=0,...,(N-1) ] $ \\
% $R_{thres}$ : The threshold for residual change\\
% $DownSample()$ : Resize to align the size of noise\\

% ---

% \textbf{residual-based}

% \For{ i from 1 to N}{
% $ res = norm( v^i - v^{(i-1)} ) $ \\
% $ res_{mask} = res > R_{thres} $ \\    
% $res_{mask}$ = $DownSample(res_{mask})$ \\
% $x^i = [x^i - x^{(i-1)} ]* res_{mask} +  x^{(i-1)}$ \\
% }
% ---

% \textbf{flow-based}

% \For{ i from 1 to N}{
% $ flow^i_{pixel} = flow( v^i , v^{(i-1)} ) $ \\
% $ flow^i_{latent} $ = $DownSample(flow_{pixel})$ \\
% $ x^i = GridSample(x^{(i-1)}, flow^i_{latent})$ \\ % gridsample?
% }
% \end{algorithm}


\subsection{Reward Feedback Learning for Controllable Video Generation}

% \begin{figure}[!t]
%    \centering
%    \includegraphics[width=1.0\linewidth]{./figures/rlhf_vis}
%        \caption{\textbf{Reward Feedback Learning for video generation}: Overview of direct reward feedback optimizing algorithm. The process involves sampling $x_T$ and denoising it to $x_{t+1}$ without gradients. Subsequently, we denoise $x_{t+1}$ to $x_{t}$, decode it, and compute quality and motion rewards. These rewards are then utilized to optimize the diffusion model. The optimization targets include enhancing aesthetic and technical quality (reducing artifacts) and ensuring motion (temporal consistency), as illustrated in the lower-left corner.
%        } \label{fig:rlhf}
%        \vspace{-0.3cm}
% \end{figure}

To enhance both the quality and motion consistency of the generated videos, we seamlessly integrate Reward Feedback Learning\cite{imageward} into our video diffusion model. As illustrated in the lower part of Figure \ref{fig:pipeline}, our training procedure entails the sampling of $x_T$, followed by denoising it to timestep $(t+1)$ without gradients. Subsequently, we denoise from $x_{t+1}$ to $x_t$ with gradient and predict $x_0'$. It is essential to highlight that selecting a small value for $t$ yields a more precise approximation of $x_0'$ and therefore leads to superior performance. Upon obtaining the predicted video, we assess its quality through a dual-pronged approach, considering both motion consistency and overall video quality.

To quantify the motion consistency of generated videos, we introduce the use of residual and optical flow~\cite{raft_flow} among frames as a motion field. The motion reward is then computed as the negative difference between this motion field and the motion field of the input video. The loss function for motion consistency is formulated as:
\begin{equation}
L_{motion} = - \lambda_{mr} \cdot R_{mr}(v, v') - \lambda_{mf} \cdot R_{mf}(v, v'),
\end{equation} 
where the ground-truth video is denoted as $v$, and $v'=Decoder(x_0')$ representing the predicted video. The residual-based motion reward $R_{mr}$ and flow-based motion reward $R_{mf}$ are calculated and subsequently combined with a weighted sum, contributing to the overall loss.

Another pivotal metric for video generation involves enhancing both the technical and aesthetic qualities in the output. Technical quality encompasses distortions, such as over-exposure, noise, and blur, present in the generated frames. We evaluate technical quality using the MUSIQ metric\cite{musiq} as a measure of technical quality reward.
Additionally,  to enhance aesthetic quality, we employ a reward model\cite{imageward} trained on a human-rated dataset, thereby enriching the overall aesthetic quality of the generated video. Consequently, the loss for quality is expressed as weighted sum of two quality reward:
\begin{equation}
L_{quality} = \lambda_{qt} \cdot ReLU( b_{qt} - R_{qt}( v' ) ) + \lambda_{qa} \cdot ReLU( b_{qa} - R_{qa}( v' ) ) .
\end{equation} 
Here, we compute frame-wise technical reward $R_{qt}$ and aesthetic reward $R_{qa}$, where $b_{qt}$ and $b_{qa}$ represent the upper boundaries of the reward models. $\lambda_{qt}$ and $\lambda_{qa}$ serve as weights.

We thus drive a spatio-temporal reward loss in sum of the above two losses as:
\begin{equation}
\mathcal{L}_{ST} = L_{motion} +  L_{quality}.
\end{equation} 
Then we update the model via feedback learning, as illustrated in Figure \ref{fig:pipeline}. For a more detailed description, the ST-ReFL algorithm is presented in Algorithm \ref{algorithm_rlhf}.

% \begin{algorithm}[!t]
% \caption{Reward Feedback Learning For Video Diffusion Models.}
% \label{algorithm_rlhf}
% \textbf{Notations:} Video diffusion model $w$, quality reward model $R_q$, motion reward $R_m$, motion weighted parameter. Total scheduler time steps $T$, randomly sampled timestep $t \in [T1, T2] $. Input latent $x$, output latent $x'$. \alpha is the learning rate. \\
% t \gets rand(T1,T2) \\ 
% x_T \sim \mathcal{N}(0, I) \\
% with no grad:  \\
% \For{ i from T to t+2}{ 
% x_{i-1} \gets w(x_i) \\
% }
% with grad: x_{t} \gets w(x_{t+1}) \\
% x_0' \gets x_t  \quad  // predict \\
% v_0' \gets x_0', v_0 \gets x_0   \quad // decode   \\
% L_{motion} \gets R_{m}(v_0, v_0'),L_{quality} \gets R_{q}(v_0') \\
% L \gets L_{motion} + L_{quality} \\
% \Delta \gets $\frac{\partial L}{\partial w}$ \\
% w' \gets w - \alpha \Delta  \quad // update 
% \end{algorithm}


% \section{Experiments}
% \label{exp}
% \subsection{Implementation Details}
% \textbf{DataSet Settings:} 100k video clips sourced from the Internet and 100k image-text pairs obtained from Laion \cite{schuhmann2022laion5b}.

% \textbf{Training Settings:} Our model is initialized with pre-trained weights from Stable Diffusion v1.5 \cite{Ramesh_Dhariwal_Nichol_Chu_Chen} and ControlNet \cite{zhang2023adding}. We only train the temporal layers with an 8:2 ratio of video to image rate. The resolution is set to $512\times 512$, the batch size to $16$, the learning rate to $10^{-5}$, and the total number of training steps to $10k$. The model is evaluated using three control types: canny edge maps \cite{Canny_2009}, hed edge maps \cite{Xie_Tu_2016}, and depth maps.\cite{Ranftl_Lasinger_Hafner_Schindler_Koltun_2020}. 

% \textbf{Inference Settings:} The noise initialization threshold is set to 0.1, the scale for text guidance is 10.0, the scale for video guidance is 1.5, and DDIM uses 20 sampling steps.

% \begin{figure}[!ht]
%    \centering
%    \includegraphics[width=0.99\linewidth]{./figures/long_video}
%        \caption{\textbf{Auto-Regressive Generation}: Our model is able to generate long videos auto-regressively. The first row is the first iteration, the second row is generating conditioned the last frame of the first iteration, and so on the third iteration.}\label{fig:long_video}
% \end{figure}
% %\vspace{-0.3cm}

% \subsection{Qualitative Results}
% \textbf{Generating Videos with Different Types of Controls:} We showcase three types of controls extracted from video to demonstrate our system's capacity to generate videos conditioned on various control types, as shown in Figure \ref{fig:head} and more results in supplementary material. Through experimentation, we found that depth maps provide less structural information than edge maps, resulting in more diverse video outputs. Edge maps, on the other hand, produce videos with enhanced details but a lesser degree of variability. For instance, in the first row of Figure \ref{fig:head}, we transform a human into a cartoon robot using depth map control. In contrast, using edge maps in the third row still results in a human-robot transformation, but with more intricate details retained, such as the clothing pattern.



% \textbf{Auto-Regressive Long Video Generation:} As illustrated in Section \ref{training}, we present the outcomes of auto-regressively producing videos in Figure \ref{fig:long_video}. The source video consists of 24 frames, and our objective is to convert a city at sunset into a frozen city. We generate the edited video through three iterations, each comprising eight frames. The generated video exhibits consistency across various iterations, which attests to the efficacy of our proposed approach in producing long videos through auto-regression based on the last frame of the previous iteration.
% % Our model can handle a large variety of video input, static background, moving camera, fast-motion, long video...

% % Despite a slight drop in frame consistency, the generated frames remain consistent enough to be considered satisfactory. These findings provide evidence for the effectiveness of our approach in generating videos from control maps and captioned prompt.
% % We also evaluated our model by generating videos without providing any prompts. The results show that our model can generate consistent frames from the control maps alone. However, without the text prompts, the generated videos may not align with the original text, resulting in lower CLIP similarity scores.

% \subsection{Comparison with Previous Methods}
% We compare our results with Gen-1 \cite{esser2023structure} and Text2Video-Zero \cite{khachatryan2023text2video} that have the same settings that generating videos with additional controls. Gen-1's results are obtained by running its product and Text2Video-Zero from their open-source code.

% \textbf{Qualitative Comparison:} To demonstrate the superior performance of our model compared to others, we chose a video with significant changes in motion. As shown in Figure \ref{fig:comp4}, the first row depicts the original video, from which we extracted depth maps and used a prompt 'a dog running through a field of poles, cyberpunk style' to create a style transfer video. In the second row, we present the most consistent and text-aligned video generated by our model. The result of Gen-1, shown in the third row, are less consistent and lack details of the dog. The last row exhibits the results of Text2Video-Zero, which fails to maintain consistency, as pointed out by the red circles. More Comparison will be shown in supplementary material.

% % the prompt in the original video is 'a dog running through a field of poles'. We add a 'cyberpunk style' to generate a style transfer video conditioned on depth maps. The first row is the original video and the second row is ours, which is the most consistent and text-aligned video that aligns with the original.  The result from Text2Video-Zero(the last row) fail to generate consistent result.
% % we provide a prompt 'a robot riding a motor in the sky' to change the subject of the man to a robot. We notice that results from Text2Video-Zero generate flickering results and the robot disintegrates after several frames. Gen-1 results generate a more consistent video while the man is not turned into a robot. Compared to them, ours is the most consistent result that aligns with the prompt.

% \begin{figure}[!ht]
%    \centering
%    \includegraphics[width=0.99\linewidth]{./figures/comp4}
%        \caption{\textbf{Qualitative Comparison:} We choose a hard case of a fast moving dog. Gen-1's result falls short of generating a detailed dog, whereas the result produced by Text2Video-Zero yields inconsistency of a dog. Ours exhibits a superior caliber compared to the aforementioned alternatives.}\label{fig:comp4}
% \end{figure}
% %\vspace{-0.2cm}


% % As shown in Figure , the prompt in the original video is 'a dog running through a field of poles'. We add a 'cyberpunk style' to generate a style transfer video. The first row is the original video and the second row is ours, which is the most consistent and text-aligned video that aligns with the original. Both other two methods either have problems with text alignment, or subject (the dog) consistency. 
% % Another case in Figure \ref{fig:comp1} shows the same result.
% % As for the moving camera case in Figure \ref{fig:comp5}, the given prompt is 'a robot riding a motor on the sky'. Our results achieve greater consistency in fast-motion video with a moving camera. Gen-1 also successfully generates consistent video while it fails to generate the subject 'robot' and its background is not consistent. Text2Video-Zero fails to generate a complete robot after a few frames. Another case for real video generation in Figure \ref{fig:comp2} also show the same result.

% % As for the second case \ref{fig:comp3}, the prompt is 'an alien jumping over the fence
% % ', this is a video that the camera is moving, the flickering of background of Gen-1 and ours is as good, while the Text2Video-Zero fails in moving camera. As for the subject 'alien', our result is still consistent in difference frames while two previous methods vary.

% \textbf{Quantitative Comparison:}
% We adopt depth maps from 20 video clips from Davis \cite{davis_2017} and in-the-wild videos, which are used to generate videos based on a given text prompt. To assess consistency, we measured \textbf{the depth map errors} between input and output videos. To evaluate text alignment, we calculated the cosine similarity between the X-CLIP \cite{ni2022expanding} video embeddings for the output videos and text embeddings for the given prompts. As presented in Table \ref{tab:Quantitative}, all methods displayed strong text alignment. Our method yielded the least depth map errors compared to the other two.

% % For \textbf{Structure Align}, we compute For \textbf{Frame Consistent}, we compute cosine similarity between CLIP image embeddings of all frames in the generated video.  
% \textbf{User Study:} 18 participants were surveyed to evaluate the textual alignment and consistency of the generated videos by utilizing a rating scale ranging from 1 to 5. The data presented in Table \ref{tab:Quantitative} indicates that our model yields videos that demonstrate greater consistency aligned the quantity result of depth error findings, with the text alignment score exhibiting comparable results.

% \begin{table*}[ht]
% \centering
% \caption{Comparison of quantitative and user study with existing methods for T2V conditioned on depth maps in terms of text alignment and consistency.}
% \label{tab:Quantitative}
% \begin{tabular}{l|cc|cc}
% \hline
% Type & Text Align $\uparrow$ & Dep Errors  $\downarrow$  & Text Align(User) $\uparrow$ & Consis(User)  $\uparrow$   \\
% \hline
% % Image ControlNet \cite{zhang2023adding}  & 0.253 & 0.114  & -  & -\\
% Gen-1 \cite{esser2023structure} & 0.252 & 0.112 & 4.25 & 3.89  \\
% Text2Video-Zero \cite{khachatryan2023text2video} & 0.255 &0.139 & 3.68 & 3.21  \\
% Ours & 0.259 & \textbf{0.091} & 4.18 & \textbf{4.18} \\
% \hline
% \end{tabular}
% \vspace{-0.4cm}
% \end{table*}

% \subsection{Ablation Study of Residual-based Noise Initialization}
% % \begin{figure}[!ht]
% %    \centering
% %    \includegraphics[width=0.99\linewidth]{./figures/zeroshotVStraining}
% %    \caption{The first row is the origin video. We generate the video with the captioned prompt from origin video. The second row is generating without any strategy, which is totally unconsistent. The third row is adding residual-based noise initialization, which can reduce the flickering and bring more consistency. The fourth row is adding spatial-temporal self-attention, which brings a lot of improvement to the model.(Only the scene is flickering and the background change little). The last row shows the most perfect video(no flickering) after training.}\label{fig:zeroshotVStraining}
% % \end{figure}
% % \textbf{}
% % The concept of residual-based noise initialization is to only modify the pixel difference between consecutive frames in order to promote stability in unchanged pixels. 
% We analyze the effects of three types of noise: identical noise (threshold=1.0), distinct noise (threshold=0.0), and motion-enhanced noise (threshold=0.1). It is important to note that this threshold also regulates the smoothness of the resulting video. As shown in Figure \ref{fig:init_thres2}, when there is no residual control, the background flickers, as seen in the second row. For example, the water changes color frequently. The third row displays the threshold we selected, which effectively balances consistency and smoothness to produce satisfactory results. The final row shows the consequence of using the same noise for each frame, a smooth video, but with severe artifacts. Overall, incorporating residual-based noise can introduce motion from the input video, resulting in videos with reduced flickering and better consistency.

% % As for spatial-temporal attention, it enable the model to do fine-grained cross-frame interaction, which leads to better consistency.
% % As shown in Figure \ref{fig:zeroshotVStraining}. In zero-shot setting, we sample a random frame-independent noise, we can see that the result is inconsistent both background and foreground. By adding the residual-based noise, we get a relatively better result with the background more consistent and less flickering. 
% % We then add the spatial-temporal attention, as shown in the third row, each frame has somewhat consistent but the flickering is very serious.(The background and the foreground change across frames if you looks the images more seriously). By combing both, we get a better result with less flickering in background and more consistent. 
% % We train the model to learn temporal modeling and the result at last row shows this training process is necessary to generate less or no flickering video. (the background still consistent unlike other zeroshot cases)

% \begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.99\linewidth]{./figures/init_thres2}
%    \caption{\textbf{Ablation Study of Different Thresholds: }We present three thresholds: 0.0, 0.1 and 1.0. Random noise(thres=0.0) allows for large changes but may result in flickering (e.g. the wave turning across frames). Same noise(thres=1.0) for each frame leads to smoothness and artifacts. Residual-based noise is a good trade-off for both changeable and consistent. } \label{fig:init_thres2}
% \end{figure}
% \vspace{-0.3cm}

% % \begin{table}[ht]
% % \centering
% % \caption{User Study}
% % \label{tab:Quantitative}
% % \begin{tabular}{|l|ccc|}
% % \hline
% % Type &   \\
% % \hline
% % Gen-1 \cite{esser2023structure} & 0 & 0   \\
% % Text2Video-Zero \cite{khachatryan2023text2video} & 0 &0 \\
% % Ours & 0 & 0\\
% % \hline
% % \end{tabular}
% % \end{table}
% % We used 50 videos captioned with BLIP \cite{Li_Li_Xiong_Hoi} from the DAVIS dataset. We extract the control maps from the origin video and use the corresponding prompt to re-generate the video with 12 frames. To evaluate the quality of our generated videos and their alignment with the input text, we used two metrics: text alignment and frame consistency. For text alignment, we compute the cosine similarity between the CLIP \cite{clip2021} image embedding of each frame and its corresponding CLIP text embedding. For frame consistency, we compute cosine similarity among CLIP image embeddings of all frames in the generated video. However, note that these metrics are not perfect and may not always capture all aspects of video quality, such as flickering, and we only compare with an open source model and a baseline that generate frames independently. As shown in Table \ref{tab:Quantitative}, the origin video has high text alignment and frame consistency. Each method generates text-aligned video as the origin video. 
% % Compared to generating frame-by-frame or Text2Video-Zero, our approach achieves higher frame consistency.



==> mqrpwsnddnxrdszwbbrtshtcmyyqyqvh/sec/3_exp.tex <==

\section{Experiments}
\label{exp}
% \begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.9\linewidth]{./figures/long_video1}
%        \caption{\textbf{Auto-Regressive Generation}: Our model is able to generate long videos auto-regressively. The first row corresponds to the initial iteration, the second row is generated conditioned on the last frame of the first iteration, and so on for the third iteration.}
%        \label{fig:long_video}
%        \vspace{-0.3cm}
% \end{figure}



\subsection{Implementation Details}
\textbf{Dataset Settings:}~ We collect 0.1M video clips from films\protect\footnotemark[1] and caption them with BLIP\cite{BLIP} and 0.1M image-text pairs randomly sampled from LAION \cite{schuhmann2022laion5b}. 

\footnotetext[1]{Note that our model can be trained on Webvid\cite{webvid} as well, but it contains watermarks.}

\noindent\textbf{Training Settings:}~ Our training regimen commences with the fine-tuning of Stable Diffusion v1.5\cite{Ramesh_Dhariwal_Nichol_Chu_Chen}, incorporating DiffusionDB\cite{diffusiondb} and a curated dataset. This refinement aims to improve the Text-to-Image (T2I) model, which is used for initialization for Temp-UNet. The initialization of Temp-ControlNet stems from ControlNet\cite{zhang2023adding}. We train the temporal layers with mixture of video and image data. The configuration includes a resolution set at $512\times 512$, a batch size of $16$, a learning rate of $10^{-5}$, and a total of $20k$ training steps. We demonstrate the architecture with three control types: Canny edge maps\cite{Canny_2009}, HED edge maps\cite{Xie_Tu_2016}, and depth maps\cite{Ranftl_Lasinger_Hafner_Schindler_Koltun_2020}. After the first stage training, we further finetune the model with reward feedback learning, where the hyper-parameters are set as $\lambda_{mr}=1.0, \lambda_{mf}=0.02, \lambda_{qt}=0.001, b_{qt}=100, \lambda_{qt}=0.005, b_{qa}=2,$. We use DDIM to sample 20 steps and set $T_1=0, T_2=5$ during ST-ReFL training.

\noindent\textbf{Inference Settings:}~ Text guidance is scaled at 7.0 and video guidance adopts a scale of 1.5. We leverage 20 sampling steps with DDIM to speedup inference. The initialization threshold is set at 0.1 for residual-based noise prior.

\noindent\textbf{Evaluation Settings:}~ We conduct comprehensive experiments to demonstrate the effectiveness of our proposed strategies qualitatively and quantitatively. 
In the quantitative comparison, we adopt depth maps from 30 video clips from Davis \cite{davis_2017}, which are used to generate videos based on a given text prompt.  
% frame consistency / optical flow map errors
Following previous works~\cite{videocomposer}, we calculate the cosine similarity between video embeddings of the output videos and text embeddings of the given prompts with CLIP \cite{clip2021}\protect\footnotemark[2] to evaluate text alignment. 
To assess semantic consistency between different frames, we measure the similarities for frame CLIP embeddings of output videos. 
Aiming at reflecting consistency with control signals, we compute the depth map errors between input and output videos.  
Inspired by VBench, we adopt MUSIQ to evaluate frame quality objectively, targeting the distortion (e.g., over-exposure, noise, blur)presented in the generated frames. 
Furthermore, we test our model on two subjective aesthetic metrics, ImageReward~\cite{imagereward} and aesthetic-predictor\protect\footnotemark[3].
\footnotetext[2]{https://huggingface.co/openai/clip-vit-large-patch14}
\footnotetext[3]{https://github.com/LAION-AI/aesthetic-predictor}
\vspace{-0.3cm}
\subsection{Main Results}

% Gen-1's result falls short of generating a detailed dog, whereas the result produced by Text2Video-Zero yields inconsistency of a dog. Ours exhibits a superior caliber compared to the aforementioned alternatives.

\subsubsection{Controllable Video Generation.}
We showcase three types of controls extracted from video to demonstrate our system's capacity to generate videos conditioned on various control types. 
As shown in Figure \ref{fig:head}, we found that depth maps provide less structural information than edge maps, resulting in more diverse video outputs. 
Edge maps, on the other hand, produce videos with enhanced details. 
For instance, in the first row of Figure \ref{fig:head}, we transform a human into a cartoon robot using depth map control. 
In contrast, using edge maps in the third row still results in a human-robot transformation, but with more intricate details retained, such as the clothing pattern.

\begin{figure}[!t]
   \centering
   \includegraphics[width=0.99\linewidth]{./figures/compare}
       \caption{\textbf{Qualitative Comparison:} (a) Input video, (b) Animatediff, (c) Text2Video-Zero, (d) Videocomposer, (e) Ours. We showcase a challenging scenario of a fast-moving dog(left) and slow-moving(right) camel. Compared to other models, our method demonstrates superior performance in generating high-quality, temporally consistent results that accurately align with the given text prompt. }\label{fig:comp4}
\vspace{-0.3cm}
\end{figure}


\begin{table}[t]
\centering
\caption{Comparison with other models. ``Img-Re'' is short for ImageReward and ``Aes-pred'' refers to Aesthetic-predictor.}
\small
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|cc|c|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{CLIP Metrics} $\uparrow$} & \textbf{Map Errors} $\downarrow$ & \multicolumn{3}{c|}{\textbf{Frame Quality} $\uparrow$} & \multicolumn{3}{c}{\textbf{User Study} $\uparrow$} \\
                       & prompt      & frames      & depth        & MUSIQ & Img-Re & Aes-pred & Text-Align & Consistency & Quality \\ \midrule
\textbf{Text2video-Zero~\cite{text2video-zero1}}        &       0.281        &       \textbf{0.964}        &    0.110        &   71.0    &       0.531      &        5.38          &     3.4       &     3.0        &     2.8    \\
\textbf{VideoComposer~\cite{videocomposer1}}           &       0.272           &       0.937       &      0.149           &    52.8   &       -0.002      &           4.60          &      3.1      &       3.6      &    2.9     \\
\textbf{AnimateDiff~\cite{animatediff1}}            &          0.274         &        0.958            &          0.097        &     59.6   &      0.67       &          \textbf{5.79}           &      3.8      &      4.0       &  4.0        \\
\textbf{Control-A-Video}      &  \textbf{0.290}          & 0.959      & \textbf{0.089}              & \textbf{73.3}          & \textbf{1.03} &  5.73                   &     \textbf{4.4}       &       \textbf{4.5}      &       \textbf{4.2}  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main_result}
\vspace{-0.4cm}
\end{table}

% \subsubsection{Auto-Regressive Long Video Generation}
% As illustrated in Section \ref{training}, we present the outcomes of auto-regressive video generation in Figure \ref{fig:long_video}. 
% The source video consists of 24 frames, and our objective is to convert a city at sunset into a frozen city. 
% We generate the edited video through three iterations, each comprising eight frames. 
% The subsequent video clips are produced auto-regressively based on the last frame of the previous iteration. 
% The generated video exhibits consistency across various iterations, which attests to the efficacy of our first-frame conditioning approach.

\subsubsection{Qualitative Analysis.}
\footnotetext[1]{We use our fine-tuned T2I model as the initialization of AnimateDiff.}
Control-A-Video can incorporate various control signals, such as depth maps, enabling it to naturally generalize to video editing and video style transfer. 
We conduct qualitative comparison on video editing with other three typical models, including Text2video-Zero~\cite{text2video-zero1} performing zero-shot video editing, VideoComposer~\cite{videocomposer1} which is a controllable video generation method, and AnimateDiff \cite{animatediff1}\protect\footnotemark[1] for animating personalized T2I models. 
% These models have similar settings for generating videos with additional controls. 
% To demonstrate the superior performance of our model compared to others, we choose videos with significant movement ranges to evaluate, which are difficult to generate. 
% More visualization cases can be found in supplementary material.
As shown in Figure \ref{fig:comp4}, the first row depicts the original video, from which we extract depth maps and use new prompts to create a style transfer video. 
In the second row, although the results of AnimateDiff have consistent subjects, the background in the first case has too much noise, which affects the visual quality. 
The third row exhibits the results of Text2Video-Zero, which fails to create a correct style and the dog in the first case is blurry. 
As for Videocomposer, it can't maintain consistency of the dog in the first case and its style is unrelated. 
In the last row, we present the videos generated by our model, which is most clear, consistent and text-aligned. 
More Comparison will be shown in supplementary material.


\begin{figure}[!t]
   \centering
   \includegraphics[width=\linewidth]{./figures/noise}
       % \caption{Qualitative ablation study of the motion-adaptive noise prior. (a) Input video, (b) Video without motion prior, (c) Video with Optical Flow-based motion prior, (d) Video with Residual-based motion prior. As shown, the generated video without any motion prior (b) exhibits severe flickering artifacts, both in the background and the subject. In contrast, when using the Optical Flow-based motion prior (c) or the Residual-based motion prior (d), the generated videos maintain better temporal consistency, with stable backgrounds and coherent subject motion over time. } 
       \caption{ \textbf{ Ablation study of motion-adaptive noise prior.} (a) Input video. (b) Without motion prior, exhibiting flickering and artifacts. (c) With Optical Flow-based prior, maintaining consistency. (d) With Residual-based prior, stable background and coherent subject motion.}
       \label{fig:noise}
       \vspace{-0.3cm}
\end{figure}

\begin{table}[!t]
\centering
\caption{Quantitative ablation comparison for our noise initialization strategies in the first training stage. The baseline indicates the model trained with depth maps as control. RNI and FNI correspond to pixel residual-based and optical flow-based noise initialization.}
\begin{tabular}{l|cc|c|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{CLIP Metrics} $\uparrow$} & \textbf{Map Errors} $\downarrow$ & \multicolumn{3}{c}{\textbf{Frame Quality} $\uparrow$}           \\
                                & prompt               & frames              & depth               & MUSIQ         & Img-Re    & Aes-pred \\ \midrule
\textbf{Baseline}               & 0.278                & 0.950               & 0.090               & \textbf{70.2} & 0.593          & 5.41                \\
\textbf{+RNI}                   & 0.284                & 0.952               & 0.089               & 69.3          & 0.737          & 5.49                \\
\textbf{+FNI}                   & \textbf{0.288}       & \textbf{0.953}      & \textbf{0.086}      & 67.1          & \textbf{0.787} & \textbf{5.52}       \\ \bottomrule
\end{tabular}
\label{tab:noise_ablation}
\vspace{-0.3cm}
\end{table}

\vspace{-0.3cm}
\subsubsection{Quantitative Comparison.} 
We conduct comparison with other end-to-end models on the 30 video clips from Davis. 
As shown in Table \ref{tab:main_result}, our model outperforms previous models in four out of six metrics. Control-A-Video achieves the highest prompt clip score and exhibits the lowest depth map errors, demonstrating superior text alignment and video consistency. Especially in terms of frame quality, our model realizes an improvement of +2.3 and +0.36 points over the previous best models on the MUSIQ and ImageReward scores, respectively. The aesthetic predictor metric of our model is comparable to that of AnimateDiff. Note that Text2video-Zero secures a higher frames clip score than ours, likely attributable to its videos having smaller ranges of movement.


As for user study, 20 participants were surveyed to evaluate the textual alignment, consistency and visual quality of the generated videos by utilizing a rating scale ranging from 1 to 5. 
Our model achieves the best performance in human evaluation.

% Please add the following required packages to your document preamble:

% \subsubsection{Quantitative Analysis}
% We adopt depth maps from 20 video clips from Davis \cite{davis_2017} and in-the-wild videos, which are used to generate videos based on a given text prompt. 
% To assess consistency, we measured \textbf{the depth map errors} between input and output videos. 
% To evaluate text alignment, we calculated the cosine similarity between the X-CLIP \cite{ni2022expanding} video embeddings for the output videos and text embeddings for the given prompts. 
% As presented in Table \ref{tab:Quantitative}, all methods displayed strong text alignment. Our method yielded the least depth map errors compared to the other two.

% We further conduct a user study with 18 participants. The participants were surveyed to evaluate the textual alignment and consistency of the generated videos by utilizing a rating scale ranging from 1 to 5. The data presented in Table \ref{tab:Quantitative} indicates that our model yields videos that demonstrate greater consistency aligned the quantity result of depth error findings, with the text alignment score exhibiting comparable results.

\vspace{-0.3cm}
\subsection{Ablation Studies}
\label{sec:ablation}
% We conduct empirical ablation experiments on our proposed strategies to demonstrate the effectiveness of motion prior and feedback learning. 

\subsubsection{Motion-adaptive Noise Prior.}
\label{ablation noise}
To demonstrate that pixel residual-based and optical flow-based noise initialization (simplify as RNI and FNI) strategies boost video consistency, we perform visualization case study and quantitative comparison in the first training stage. 
Figure~\ref{fig:noise} illustrates the effect of different noise initialization strategies. 
In the second row, the bear in the first case has artifacts and the backgrounds in both cases have many flickers. 
In contrast, due to the presence of motion-adaptive noise prior, the video in last two rows are more consistent, which exhibits superior visual performance. 

As summarized in Table~\ref{tab:noise_ablation}, both noise initialization methods, RNI and FNI, improve all metrics except MUSIQ over the baseline. 
The results demonstrate that videos initialized with RNI and FNI exhibit higher prompt consistency and frame-level consistency. 
Additionally, errors in depth maps are reduced, indicating that the motion prior successfully contribute to maintaining the structure of the source video. 
Notably, in terms of aesthetic metrics, RNI and FNI enhance the ImageReward score by 0.144 and 0.194, respectively. 
The ablation study for the threshold of residual-based noise initialization is detailed in the Appendix.

% For residual-based noise initialization, we set the $R_{thres}$ in Algorithm~\ref{algorithm} to 0.1. 
% We analyze the effects of three types of initial noise: identical noise (threshold=1.0), distinct noise (threshold=0.0), and motion-enhanced noise (threshold=0.1). 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \noindent\textbf{Threshold of residual-based noise initialization. }
% We analyze the effects of three types of initial noise: identical noise (threshold=1.0), distinct noise (threshold=0.0), and motion-enhanced noise (threshold=0.1). 
% It is important to note that this threshold also regulates the smoothness of the resulting video. 
% As shown in Figure \ref{fig:init_thres}, in the second row, when there is no residual control, the background is prone to flickering, such as water color. 
% The third row corresponds to the threshold we select, which effectively balances consistency and smoothness to produce satisfactory results. 
% The final row displays the consequence of using the same noise for each frame, a smooth video, but with severe artifacts. 
% Overall, incorporating residual-based noise can introduce motion from the input video, resulting in videos with reduced flickering and better consistency.

% \begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.7\linewidth]{./figures/init_thres5}
%    \caption{Ablation Study of Different Thresholds} \label{fig:init_thres}
%    \vspace{-0.3cm}
% \end{figure}


\begin{figure}[!t]
   \centering
   \includegraphics[width=\linewidth]{./figures/rlhf_compare}
        \caption{\textbf{Qualitative ablation study of ST-ReFL optimization}. Three examples before and after ST-ReFL show improved consistency and quality through feedback tuning from motion and quality reward models.}
       \label{fig:rlhf_compare}
       \vspace{-0.3cm}
\end{figure}

\subsubsection{Spatial-Temporal Reward Feedback Learning.}
We integrate four reward feedback signals into controllable video generation, two of which are designed to improve video quality and the other two for enhancing consistency. 
As depicted in Figure \ref{fig:rlhf_compare}, we provide a qualitative comparison for the model with and without ST-ReFL training. 
Take the first row as an example, the dog has clear texture and its facial features appear lifelike after ST-ReFL training, indicating ST-ReFL improves frame quality and aesthetic effect. 
In the second row, before ST-ReFL training, there are some color changes on the floor and the clothes of the person. 
In the third rows, there are some artifacts on the car wheel. 
Nonetheless, our final model delivers consistent videos of high quality, as evidenced by the results.

To investigate the individual impact of each reward signal, we conduct quantitative ablation experiments during the second stage training, systematically omitting one signal at a time. 
The results are shown in Table \ref{tab:ablation_reward}. 
Compared to the results of the first four lines, our complete model achieves a balance across all metrics and gains the best overall performance. 
Specifically, as observed in the first row of the table, the absence of the aesthetic reward compromises the model’s performance on video clip metrics and frame-level aesthetic evaluation. 
The second line highlights the results without technical reward are the worst on MUSIQ, which indicates technical reward plays an important role in frame quality. 
In the third line, when removing residual reward, the depth error and frame quality get worse. 
Comparing results of the last two lines, optical flow reward makes a significant improvement on motion consistency and ImagReward score.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


\begin{table}[t]
\centering
\caption{Ablation studies of different reward signals. The best scores are in \textbf{bold} and the second best scores are \ul{underlined}.}
\label{tab:ablation_reward}
\begin{adjustbox}{max width=\textwidth}
\small
\begin{tabular}{l|cc|c|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}}  & \multicolumn{2}{c|}{\textbf{CLIP Metrics} $\uparrow$} & \textbf{Map Errors} $\downarrow$ & \multicolumn{3}{c}{\textbf{Frame Quality} $\uparrow$}          \\
                                 & prompt               & frames              & depth                & MUSIQ         & Img-Re   & Aes-pred \\ \midrule
\textbf{w/o Aesthetic reward}    & 0.288                & 0.955               & {\ul 0.089}           & {\ul 74.4}    & 0.897         & 5.70                \\
\textbf{w/o Technical reward}    & 0.289                & {\ul 0.958}         & \textbf{0.086}          & 70.7          & 0.983         & 5.62                \\
\textbf{w/o Residual reward}     & \textbf{0.292}       & {\ul 0.958}         & 0.093                  & 72.4          & {\ul 0.996}   & 5.69                \\
\textbf{w/o Optical flow reward} & 0.286                & 0.957               & 0.094                  & \textbf{75.6} & 0.866         & \textbf{5.75}       \\
\textbf{Control-A-Video (Ours)}  & {\ul 0.290}          & \textbf{0.959}      & {\ul 0.089}              & 73.3          & \textbf{1.03} & {\ul 5.73}          \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-0.4cm}
\end{table}

% \subsubsection{Latent First-frame Conditioned Controller}
% \label{ablation first}
% Our first-frame conditioning strategy provides content prior for video generation, encouraging subsequent frames to keep object consistency with the first frame. 
% Because the initial frame from text-to-image process can achieve high quality and text-aligned easily, two-stage video generation facilitates semantic alignment with prompt compared with generating an entire video directly. 
% Figure~\ref{fig:first} compares the results with and without the first-frame conditioning strategy. 
% In this case, the caption describes the bus is red and blue, but the result without first-frame conditioning produces a bus in wrong color. 
% Moreover, our model can generate snowflakes in the video background, which is consistent with ``a snowy day''. 
% According to Table~\ref{table:quan}, the first-frame conditioned controller brings boost in text alignment, from 0.238 to 0.262, and reduces depth errors, from 0.149 to 0.086, over the baseline. 
% Compared with noise initialization strategies, first-frame conditioning plays a more important role in text alignment and depth consistency.

% \begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.7\linewidth]{./figures/first_a1}
% %   \includegraphics[width=0.99\linewidth]{./figures/first_b1}
%        \caption{Qualitative ablation study of the first-frame conditioned controller (FFC). (a) Input video, (b) Ours w/o FFC, (c) Ours with FFC.   }
%        \label{fig:first}
% \end{figure}
% %\vspace{-0.2cm}


% \begin{table}[!t]
% \centering
% \small
% %\begin{adjustbox}{max width=0.5\textwidth}
% \begin{tabular}{l|cccc}
% \toprule
% type        & text  & frame & depth & optical flow \\ \midrule
% baseline    & 0.238 & 0.950 & 0.149 & 4.78         \\
% + FFC       & 0.262 & 0.964 & 0.086 & 4.40         \\
% + RNI       & 0.256 & 0.954 & 0.104 & 3.72         \\
% + FNI       & 0.255 & 0.954 & 0.095 & 3.66         \\
% + FFC + RNI & 0.264 & 0.960 & 0.092 & 4.12         \\
% + FFC + FNI & 0.261 & 0.965 & 0.088 & 4.09         \\ \bottomrule
% \end{tabular}
% %\end{adjustbox}
% \caption{Quantitative comparison for our strategies in terms of text alignment, frame similarity, depth map error and optical flow map error. The baseline indicates the model trained with depth maps as control. FFC means first-frame conditioned controller. RNI and FNI correspond to pixel residual-based and optical flow-based noise initialization.}
% \label{table:quan}
% \vspace{-0.3cm}
% \end{table}



==> mqrpwsnddnxrdszwbbrtshtcmyyqyqvh/sec/4_conclusion.tex <==
\vspace{-0.3cm}
\section{Conclusion}
% In this paper, we propose a controllable T2V framework that is capable of generating videos conditioned on text prompts and control maps. 
% With the proposed motion-adaptive noise initialization and first-frame conditioning strategies, we introduce motion prior and content prior to promote video consistency. 
% After temporal learning in a small video dataset, our model can generate coherent, text-aligned, long videos. 
% While our method achieves impressive results, it still has some known limitations. 
% For example, our T2V model relies on a T2I model and shares the same bad cases. 
% % If the input control maps extracted from another model is not consistent, it also brings errors to the generated videos. 
% In the future, it's worth conducting research on the stability and controllability of the video generation models.

In this paper, we introduce a controllable Text-to-Video (T2V) framework for generating videos based on text prompts and control maps. Our framework leverages content prior extracted from an initial frame, facilitating the transition from the image to video domain. Additionally, we enhance temporal consistency by employing motion prior derived from residual/optical flow initialization. Moreover, our Spatio-Temporal Reward Feedback Learning algorithm optimizes the model with dedicated reward models, resulting in significant improvements in both video quality and motion coherence. Our combined strategies offer innovative avenues for enhancing the quality and controllability of diffusion-based video synthesis through prior initialization and reward feedback learning.



==> mqrpwsnddnxrdszwbbrtshtcmyyqyqvh/sec/5_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/5_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
